Only One Relation Possible? Modeling the Ambiguity in Event Temporal Relation Extraction

Event Temporal Relation Extraction (ETRE) aims to identify the temporal relationship between two events, which plays an important role in natural language understanding. Most previous works follow a single-label classification style, classifying an event pair into either a specific temporal relation (e.g., \textit{Before}, \textit{After}), or a special label \textit{Vague} when there may be multiple possible temporal relations between the pair. In our work, instead of directly making predictions on \textit{Vague}, we propose a multi-label classification solution for ETRE (METRE) to infer the possibility of each temporal relation independently, where we treat \textit{Vague} as the cases when there is more than one possible relation between two events. We design a speculation mechanism to explore the possible relations hidden behind \textit{Vague}, which enables the latent information to be used efficiently. Experiments on TB-Dense, MATRES and UDS-T show that our method can effectively utilize the \textit{Vague} instances to improve the recognition for specific temporal relations and outperforms most state-of-the-art methods.

==> chapters/approach_v1.tex <==
\section{Our Approach}
% \begin{figure*}[pt]
%     \center
%     \includegraphics[width=0.95\textwidth]{fig/Model_horizon.pdf}
%     \caption{The overview of our architecture. $h_{e_1,e_2}$ is the representation of the event pair $(e_1,e_2)$. The abscissa of the histogram represents 5 well-defined relations and the threshold. CR is the abbreviation of confusion relation.}
%     \label{fig:architecture}
% \end{figure*}

\begin{figure}[pt]
    \center
    \includegraphics[width=0.48\textwidth]{fig/Model_vertical.pdf}
    \caption{The overview of our architecture. $h_{e_1,e_2}$ is the representation of the event pair $(e_1,e_2)$. The abscissa of the histogram represents 5 well-defined relations and the threshold. CR is the abbreviation of confusion relation.}
    \label{fig:architecture}
\end{figure}

Figure~\ref{fig:architecture} shows the overview of our approach. Given an input text $\mathbf{S}$ and an event pair $(e_1, e_2)$, where both $e_1$ and $e_2$ are in $\{w_i|i\in[1, n]\}$. The task of temporal relation extraction is to predict the temporal relation $r\in \tilde{R} = R\cup \{Vague\}$ between $e_1$ and $e_2$. $\tilde{R}$ is the union of a well-defined temporal relations set $R$ and a special relation \textit{Vague}.

\red{xxxx} % 3.1 --3.4 都subsection 有点太密集了。 3.5 又太大块了。如果重心在 training objective哪里，前面是不是可以合并一下？
\subsection{Encoder Module}
% \red{First describe what Encoder does, then the details.}
In our work, we adopt pre-trained language model BERT and RoBERTa as the encoder. Take the text sequence $\mathbf{S} = [w_1, w_2, ..., w_n]$ and an event pair $(e_1, e_2)$ as input, it computes the contextualized representation of the event pair. Following \citet{zhong2021frustratingly}, we insert typed markers at the input layer to highlight two event mentions $e_1$ and $e_2$. So we define typed markers as <E1:L>, <E1:R>, <E2:L>, <E2:R>, and apply them at the sides of $e_1$ and $e_2$ respectively in the given text. In addition, inspired by \citet{DBLP:conf/emnlp/WaddenWLH19}, we add cross-sentence context, 1 sentence before and after the given text, expecting pre-trained language models to capture more comprehensive information. 
% \red{I don't  think the \textit{symmetry trick} should be here. Maybe, we could put them in the experiment settings?} 
With the new sequence $\tilde{\mathbf{S}}$, we feed it into the encoder and obtain the event pair representation:
\begin{equation}
    \mathbf{h}_{e_1,e_2} = MLP_1([\mathbf{x}_{\hat{e_1}}||\mathbf{x}_{\hat{e_2}}])
    \label{eq:event_pair}
\end{equation}
where $\mathbf{x}$ is the output representation, $\hat{e_i}$ is the indices of $e_i$ in $\tilde{\mathbf{S}}$, [·||·] is the concatenation operator, and $MLP_1$ is a multilayer perceptron.

\subsection{Classifier Module}

\paragraph{Baseline Classifier}
% \red{This module does not appear in the Figure 1}

Given the representation of an entity pair $(e1, e2)$ computed by Equation~\ref{eq:event_pair}, we calculate the probability distribution of relation $r$ by $MLP_2$ and softmax activation. This can be formulated as:
\begin{equation}
    P(\tilde{R}|e_1, e_2) = softmax(MLP_2(\mathbf{h}_{e_1,e_2}))
\end{equation}
where $P(r_i|e_1, e_2)$ denotes the probability of relation $r_i \in \tilde{R}$ exits between $e_1$ and $e_2$. We use the cross-entropy loss for training. The relation with the highest probability is predicted as the final decision when inferring.


\paragraph{Multi-Label Classifier}
% \red{Instead of  choosing one relation from the $\hat{R}$, our model predicts the probability of each relation independently. XXXX}
For a better representation of \textit{Vague}, we use multi-label classification method as our classifier. Different from single-label classification, which directly chooses the relation of the highest probability from $\tilde{R}$, our model make prediction on the probability of every well-defined relation $r\in R$ independently, and decides whether it could be the temporal relation between the given event pair. If only one relation is chosen, we determine it as final prediction of the temporal relation between the event pair. Otherwise, we think the temporal relation is \textit{Vague}.

\paragraph{\cyan{Loss Function}}
% hyt: loss function这一节可以放进classification module吗
Given an event pair, let $POS$ is the set of all possible relations between them while $NEG$ is the set of all impossible relations. To make a correct prediction, our classifier is expected to give higher probablity to all relations in $POS$ than relations in $NEG$. Inspired by \citet{zhou2020documentlevel}, we use a learnable, adaptive threshold for different event pairs to decide what $POS$ and $NEG$ should be composed of, and use the standard cross entropy loss to encourage the probability of relations in $POS$ to be higher than threshold $T$ while that in $NEG$ to be lower. Therefore, the loss functions are formed as:
\begin{equation}
    \small
    L_{POS} = -\sum_{r\in POS}log(\frac{exp(P(r))}{\sum_{r\in POS}exp(P(r))+exp(T)}) \\
\end{equation}
\begin{equation}
    \small
    L_{NEG} = -log(\frac{exp(T)}{\sum_{r\in NEG}exp(P(r))+exp(T)})
\end{equation}
\begin{equation}
    \small
    L = L_{POS} + L_{NEG}
\end{equation}

% Notice that, $POS$ of \textit{Vague} comes from the probability distribution provided by the model, and can not fully represent the true underlying composition of \textit{Vague}. To avoid the error propagation, if $P\{r_i|e_m, e_n, r_i\in POS\} > V_{mn}$, we do not further encourage the probability of $r_i$ to be higher. Besides, some potential relations may be ignored by the current model and not be considered into $POS$, so we set $NEG$ to empty to avoid decreasing the probability of any potential candidate relations. For event pairs whose gold label are \textit{Vague}, the loss function is formed as:
% \begin{equation}
%     \label{eq:vague loss}
%     \small
%     L_3 = -\sum_{r\in POS \atop \land P(r)<V}log(\frac{exp(P(r))}{\sum_{r\in POS\atop \land P(r)<V}exp(P(r))+exp(V)}) \\
% \end{equation}

% Since the model provides nearly random probability distribution at the first few steps of the training process, we set a weight hyperparameter $w$ and a linear increasing rate hyperparameter $\alpha$ to Equation~\ref{eq:vague loss}. The final weight should not exceed $w$ due to the uncertainty in $POS$. The final loss function is computed as:
% \begin{equation}
%     L = L_1 + L_2 + MIN(\alpha*w, w)*L_3
% \end{equation}


\subsection{Training Objective}
% \red{Introducing dynamic threshold here, and then describe the objective in Equations. }

% \red{The discussion of Vague should also be put here, to explain how to construct POS and NEG.}

% As mentioned in Section~\ref{sec:intro}, the underlying meaning of \textit{Vague} is likely to be ignored if the model simply uses single-label classification to make predictions. Instead, if we convert the task into a multi-label classification task, and treat \textit{Vague} as the scenarios when there are multiple possible temporal relationships between an event pair, we can utilize the latent information behind \textit{Vague} to help model better capture the patterns of well-defined relations.  

% \subsubsection{Multi-label Classification}

% The benefit of multi-label classification is that labels may simultaneously belong to an event pair and thus make it possible to model the meaning of \textit{Vague}. In order to intuitively judge which temporal relation subset of $R$ is likely to be the relationships between $e_1$ and $e_2$, a threshold is needed to determine the probability lower limit of the relations being selected. Following \citet{zhou2020documentlevel}, we use a learnable, adaptive threshold for different event pairs and make more suitable and confident decisions on the selection of candidate temporal relations. Specifically, for every event pair $(e_m, e_n)$, our model will calculate a unique threshold value, denoted as $V_{mn}$, and expect $P(r_i|e_m, e_n, r_i\in R\cap r_i\in POS_{mn}) > V_{mn}$ and $P(r_i|e_m, e_n, r_i\in R\cap r_i\in NEG_{mn}) < V_{mn}$, where $POS_{mn}/NEG_{mn}$ is the set of the temporal relations which are possible/impossible to be the ones between event pair $(e_m, e_n)$.

% \subsubsection{Composition of \textit{Vague}}
\label{sec:pos_1}
It is important to decide which temporal relations belong to $POS$ and which belong to $NEG$ during training process. For event pair whose gold temporal relation is a well-defined relation $r\in R$, it is easy to assert that $POS_r=\{r\}$ and $NEG_r=R/\{r\}$. While for event pair whose temporal relation is labeled as \textit{Vague}, we lack the information to identify what relations are the possible ones for sure. However, thanks to the relation probability distribution $P(R|e_1, e_2)$ provided by the model, we can temporarily assume the composition of $POS_{Vague}$ with the following considerations:

\textbf{Top2 relations in probability ranking.} After a period of pre-training with well-defined relations, we can assume that our model has the ability in providing a relatively accurate probability of each temporal relation of an event pair. According to the definition of \textit{Vague}, it means that there are at least two temporal relationships that could be between an event pair. Therefore, we adopt the result of the probability distribution and consider the highest two relations in probability ranking, $r_{fir}$ and $r_{sec}$, are most likely to be ones between this event pair.

\begin{table}[t!]
    \centering
    \scriptsize
    % \small
    \begin{tabular}{c|ccccc}
        \toprule
        r & \textit{Before} & \textit{After} & \textit{Include} & \textit{Is included} & \textit{Simultaneous} \\
        \midrule
        \makecell[l]{$\bar{r}$} & \textit{Include} & \textit{Is included} & \textit{Before} & \textit{After} & - \\
        \bottomrule
    \end{tabular}
    \caption{Well-defined relations and their corresponding confusion relation.}
    \label{tab:confusion relation}
\end{table}

\textbf{Confusion relation of Top1 relation.}%\label{sec:confuse relation} The temporal relationships between an event pair $(e_1, e_2)$ can be represent by two time intervels ($[t_{start}^1,t_{end}^1]$ and $[t_{start}^2,t_{end}^2]$) \cite{ning2018multi}. 
The determination of a temporal relation is always based on the relations between both the start-point and end-point. \citet{ning2018multi} claims that comparisons of end-points (eg., $t_{end}^1$ vs. $t_{end}^2$) are typically more difficult than comparing start-points (eg., $t_{start}^1$ vs. $t_{start}^2$), which can be attributed to the ambiguity of expressing and perceiving durations of events in \citet{COLLFLORIT201141}. Based on this, we believe that \textit{Vague} may come from the ambiguity between the end-points relation of an event pair. For example, if it is easy to figure out $e_1$ starting before $e_2$ while hard to decide the end-point relation, annotators will have disagreement between \textit{Before} ($t_{start}^1<t_{start}^2\land t_{end}^1<t_{end}^2$) and \textit{Include} ($t_{start}^1<t_{start}^2\land t_{end}^1\geq t_{end}^2$). Here we name \textit{Before} and \textit{Include} are the \textbf{confusion relation} of each other. According to the ambiguity of end-points, table~\ref{tab:confusion relation} shows all relations $r\in R$ together with their confusion relations $\bar{r}$. Back to the composition of \textit{Vague}, as the model provides a candidate relation with the highest probability, we conjecture it is probable that the relations between the event pair could be both the highest relation in probability ranking and its confusion relation, $r_{fir}$ and $\bar{r}_{fir}$, which finally cause \textit{Vague}.

In summary, we think \textit{Vague} most likely consists of the relations with the highest probability and its confusion relation, as well as the relation with the second highest probability, so we set $POS^{init}_{Vague}=\{r_{fir}, \bar{r}_{fir}, r_{sec}\}$. Notice that, $POS^{init}_{Vague}$ comes from the probability distribution provided by the model, and can not fully represent the true composition of \textit{Vague}. To avoid the error accumulation, if the probability of $r_i$ is already higher than the threshold, we do not further encourage it to be higher. Hence, we define $POS_{Vague}$ as:
\begin{equation}
    \small
    POS_{Vague}=\{r_i|r_i\in POS^{init}_{Vague}, P(r_i)<T\}
\end{equation}

Considering that some potential relations may be ignored by the current model and not be considered into $POS_{Vague}$, we set $NEG_{Vague}$ to a empty set to avoid decreasing the probability of any potential candidate relations. Besides, since the model provides nearly random probability distribution at the first few steps of the training process, we set a weight hyperparameter $w$ that increase linearly with a rate of $\alpha$ to control the effect of the loss from \textit{Vague}. The final weight should not exceed $\bar{w}$ due to the uncertainty in $POS$. The final loss function is formulated as:
\begin{equation}
    L = \sum_{r\in R}(L_{POS,r} + L_{NEG,r}) + w*L_{POS,Vague}
\end{equation}
where $w=MIN(\alpha*\bar{w}, \bar{w})$.

\subsection{\blue{Inference}}
With the multi-label classifier, the temporal relationship of an event pair can be deduced from the probability distribution $P(R)$ and corresponding threshold $T$. Specifically, if only one relation whose probability is higher than the threshold, we consider this well-defined relation as the final prediction. While if more than one relation's probability is higher than the threshold, we think the temporal relation of the event pair is \textit{Vague}, and we can provide detailed information on exactly what relations cause the ambiguity. There are also some cases that all relations' probability are lower than the threshold, we map it to \textit{Vague} as well, which can be explained as the model does not have enough confidence in any relation for the event pair.
